CUDA-Q Logical: Retargetable Compilation for Fault-Tolerant Quantum Computing

Realizing fault-tolerant quantum computing requires mapping logical programs to heterogeneous quantum error correction (QEC) codes and diverse fault-tolerant execution models, scheduling physical resources, and coupling to real-time classical control and feedback. Specialized tools exist for each step but rely on manual composition and translation that discard assumptions and provenance, separating resource estimates from the compiler artifacts they describe, and making it difficult to validate correctness, compare architectures, or attribute costs to specific design choices. We present CUDA-Q Logical, an extensible compiler infrastructure for retargetable fault-tolerant compilation, analysis, and execution. Interoperable with CUDA-Q and other mainstream front-ends, CUDA-Q Logical progressively lowers target-independent logical programs through a constrained logical virtual machine, QEC microcode, physical gate schedules, and real-time control plans, with each layer preserving semantics and provenance, while verifying composition and resource constraints. By deriving every resource estimate directly from compiler artifacts, the framework unifies compilation and resource analysis, enabling successively refined estimates and principled cross-architecture comparison while permitting QEC codes, execution models, decoders, and hardware architectures to be introduced as modular extensions. Across workloads ranging from application-architecture studies to qLDPC surgery and detector-error-model composition, we show that schedule-derived estimates reconcile with established independent models. Crucially, this compiler-visible structure exposes cost drivers hidden by aggregate analytical formulas, carries QEC artifacts intact into simulation, and demonstrates a complete compilation pipeline for fault-tolerant quantum computing.

==> Makefile <==
PYTHON ?= python3
LATEXMK ?= latexmk
TECTONIC ?= $(CURDIR)/.tools/tectonic
ROOT := main.tex
BUILD_DIR := build

.PHONY: all pdf strict setup check check-pdf clean distclean help

all: pdf

pdf: check
	@mkdir -p $(BUILD_DIR)
	@if command -v $(LATEXMK) >/dev/null; then \
		echo "Building with latexmk"; \
		$(LATEXMK) -pdf -outdir=$(BUILD_DIR) $(ROOT); \
	elif [ -x "$(TECTONIC)" ]; then \
		echo "Building with project-local Tectonic"; \
		mkdir -p "$(CURDIR)/.tools/cache" "$(CURDIR)/.tools/config"; \
		XDG_CACHE_HOME="$(CURDIR)/.tools/cache" \
		XDG_CONFIG_HOME="$(CURDIR)/.tools/config" \
		bash scripts/run_tectonic.sh "$(TECTONIC)" "$(ROOT)" "$(BUILD_DIR)"; \
	else \
		echo "No TeX engine found. Run 'make setup' to install the verified project-local Tectonic fallback."; \
		exit 127; \
	fi
	$(MAKE) check-pdf

# Zero-warning gate for release builds; the working build tolerates layout
# warnings (overfull boxes, wrapfig collisions) that move with every edit.
strict: pdf
	$(PYTHON) scripts/check_tex_log.py $(BUILD_DIR)/main.log

setup:
	bash scripts/bootstrap_tectonic.sh

check:
	$(PYTHON) scripts/check_project.py

check-pdf:
	$(PYTHON) scripts/check_pdf.py $(BUILD_DIR)/main.pdf

clean:
	@if command -v $(LATEXMK) >/dev/null; then \
		$(LATEXMK) -c -outdir=$(BUILD_DIR) $(ROOT); \
	fi

distclean:
	@if command -v $(LATEXMK) >/dev/null; then \
		$(LATEXMK) -C -outdir=$(BUILD_DIR) $(ROOT); \
	fi

help:
	@echo "make setup      Install the verified project-local Tectonic fallback"
	@echo "make check      Validate project structure, references, labels, and citations"
	@echo "make pdf        Validate, build, and inspect build/main.pdf"
	@echo "make strict     make pdf, then fail on any remaining TeX warning"
	@echo "make clean      Remove intermediate TeX files"
	@echo "make distclean  Remove all generated TeX/PDF files"


==> sections/evals/rsa-gidney-ekera.tex <==
% \newpage

\subsubsection{RSA-2048 Gidney-Ekera Architecture}
\label{sec:results-rsa2048}
In this study, we reproduce the resource-analysis workflow for the
Gidney--Eker{\aa} RSA-2048 architecture in CUDA-Q Logical and derive resource
estimates from compiled schedules across a range of algorithmic and factory
parameters.  The reproduction expresses the workload, resource factories, and
physical architecture as compiler inputs rather than importing final estimates
from a closed-form model.  Consequently, the resulting schedules retain enough
structure to attribute runtime and physical-qubit costs to architectural
decisions.  We use this attribution to identify the boundary between
factory-limited and compute-limited execution, showing when algorithmic
parallelism reduces wall-clock time and when factory production limits that
benefit.

% \begin{wrapfigure}{r}{0.54\textwidth}
%   \begin{minipage}{\linewidth}
\begin{lstlisting}[
  style=qlx-python,
  float=!b,
  % basicstyle=\scriptsize\ttfamily,
  aboveskip=0pt,
  belowskip=0pt,
  caption={Abridged P0 RSA-2048 workload; study-local QROM, carry-runway, allocation, and cleanup helpers are elided.},
  label={lst:ge-qlx-p0}
]
import cudaq.logical as ql 

def lookup_addition(_iteration, *live):
    live = qrom_lookup(live, rows=1_023)
    live = carry_runway_add(live, piece_length=1_062)
    return qrom_unlookup(live, accesses=64)

@ql.program
def rsa2048_resource_program() -> None:
    live = allocate_rsa_workspace(register_length=2_124, address_width=10, carry_pieces=2)
    live = ql.ops.repeat(505_965, carries=live, body=lookup_addition)
    measure_and_release(live)
\end{lstlisting}
%   \end{minipage}
% \end{wrapfigure}
The Gidney--Eker{\aa} architecture reduces the quantum portion of RSA-2048
factoring to a short-discrete-logarithm computation dominated by windowed
modular exponentiation~\cite{gidney2021factoring}.  It combines windowed
arithmetic, coset padding, oblivious carry runways, and a bank of CCZ-state
factories.
Listing~\ref{lst:ge-qlx-p0} summarizes the folded P0 authoring structure.
Our compiler workload retains the paper's selected operating point, $c_{\mathrm{exp}}=c_{\mathrm{mul}}=5$,  and folds the resulting 505,965 lookup additions instead of materializing
billions of identical non-Clifford operations in the host program.

Each lookup addition is represented by two dominant submodules.  The
\emph{WindowLookup} uses the joint exponent and multiplication windows as a
10-bit address.  Unary iteration visits the 1,023 nonzero table rows and writes
the selected value into a persistent lookup bus; 64 alternating accesses retain
the discrete recurrence for measurement-based uncomputation.  The
\emph{oblivious carry-runway adder} then consumes that value through forward
majority (MAJ) and reverse unmajority-and-add (UMA) sweeps.  Keeping these
helper calls explicit is important: CUDA-Q Logical observes the typed owner dependencies,
CCZ-state demand, and structural relationships of each lookup and addition layer directly, rather than receiving only an
aggregate Toffoli count.
This compiler-visible structure allows later compilation stages to attribute resource, scheduling, and factory costs to specific program components instead of reconstructing them from analytical summaries.
% \begin{wrapfigure}{l}{0.55\textwidth}
%   \begin{minipage}{\linewidth}
\begin{lstlisting}[
  style=qlx-python,
  % basicstyle=\scriptsize\ttfamily,
  aboveskip=0pt,
  belowskip=0pt,
  caption={Abridged layered construction of the RSA-2048 device from a compiler-characterized AutoCCZ factory.},
  label={lst:ge-factory-device}
]
import cudaq.logical as ql 

# Compile the factory schedule into a P3 model that produces AutoCCZ states
factory_model = ql.compiler.factory_model(factory_schedule, produces=ql.standard.AUTO_CCZ_STATE)

# Derive the physical footprint of one compiled factory lane 
FACTORY_LANES = 28
lane = factory_model.characterization
lane_footprint = ql.architecture.PhysicalFootprint(lane.physical_unit_kind, lane.physical_units,
    "compiled AutoCCZ P3 schedule")

# Build the Gidney-Ekera architecture / device 
# Declare logical compute and state factory regions
b = ql.devices.DeviceBuilder("GidneyEkeraArch")
compute = b.logical.add_compute(capacity=COMPUTE_PATCHES, name="compute")
factory = b.logical.add_factory(produces=ql.standard.AUTO_CCZ_STATE,
    via=surface_autoccz_factory, capacity=FACTORY_LANES, name="autoccz_factory")

# Bind QEC architectures and encodings to the logical regions
compute_qec = b.qec.bind(compute, architecture=architecture)
factory_qec = b.qec.bind(factory, encoding=CODE, block_capacity=9 * FACTORY_LANES)

# Define P3 level physical resources
compute_grid = b.physical.add_resources("surface_code_patch", COMPUTE_PATCHES, **_surface_resource_options(SURFACE))
routing_pool = b.physical.add_resources("surface_code_patch", 12, **resource_options)
factory_bank = b.physical.add_resources("autoccz_factory_lane", FACTORY_LANES,footprint=lane_footprint)

# Map each QEC region to its physical resource pool
b.physical.bind(compute_qec, to=compute_grid)
b.physical.bind(compute_qec.auxiliary_regions[0], to=routing_pool)
b.physical.bind(factory_qec, to=factory_bank, factory_model=factory_model)

# Supply timing and calibration data needed by the physical model 
b.physical.set_operating_point(timing=_surface_timing(), calibration=...)

# Build the architecture
device = b.build()
\end{lstlisting}
%   \end{minipage}
% \end{wrapfigure}

The oblivious carry-runway adder partitions the working register at a
separation $c_{\mathrm{sep}}$.
Carries propagate within each piece while runway state defers communication
between pieces, allowing disjoint pieces to execute in lockstep.  Thus
$c_{\mathrm{sep}}$ bounds the longest within-piece carry chain and determines
the number of pieces, $\lceil n/c_{\mathrm{sep}}\rceil$.  The coset padding
$c_{\mathrm{pad}}$ supplies slack against modular runoff and is included in
each piece.  The ancillary cost convention used by this implementation gives
$c_{\mathrm{pad}}=38$ for RSA-2048.  At the paper operating point
$c_{\mathrm{sep}}=1024$, the working register is consequently represented by
two 1,062-bit pieces.  Together, $c_{\mathrm{sep}}$ and
$c_{\mathrm{pad}}$ determine the local adder width, runway storage, and
reaction-depth contribution of a lookup addition.

\begin{figure*}[b]
  \centering
  \includegraphics[width=0.47\textwidth]{figures/08-ge-wall-clock-sweep.pdf}
  \includegraphics[width=0.47\textwidth]{figures/08-ge-physical-qubits-sweep.pdf}
  \caption{RSA-2048 tradeoffs across CCZ factory-lane
    counts and carry-runway separations. From left to right: single-run
    wall-clock time and physical-qubit footprint.}
  \Description{Two line plots. Left: single-run wall-clock time in hours
    versus the number of CCZ factory lanes for three carry-runway separations;
    each curve falls and then plateaus. Right: physical-qubit footprint versus
    factory lanes for the same separations, rising linearly.}
  \label{fig:ge-factory-csep-sweep}
\end{figure*}

\begin{wraptable}{r}{0.55\linewidth}
    \centering
    \caption{Default-point cross-check at
      $c_{\mathrm{sep}}=1024$ and 28 factory lanes.
      The independent column reconstructs only quantities
      defined by the source model; compiler-internal schedule
      structure is reported separately in the text.}
    \label{tab:ge-reconciliation}

    \footnotesize
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{@{}lrr@{}}
      \toprule
      Quantity
        & \shortstack{CUDA-Q Logical\\schedule}
        & \shortstack{Independent\\reconstruction} \\
      \midrule
      Wall-clock time (h)
        & 5.046228
        & 5.046228 \\
      \midrule
      Physical qubits
        & 19,252,128
        & $19{,}248{,}768 + 28 \times 120$ \\
      \bottomrule
    \end{tabular}
  \end{wraptable}
Listing~\ref{lst:ge-factory-device} opens the factory-to-device provenance
chain. A reusable model is derived from the detailed factory's P3 schedule;
its characterized physical units become the footprint of one factory-lane
resource. The user-specified \texttt{DeviceBuilder} code separately declares the logical compute and
28-lane factory regions, refines them through QEC, and binds them to compute,
routing, and factory resource pools before attaching the selected operating
point.
The CUDA-Q Logical implementation represents the application as the folded P0 helper-call
graph shown in Listing~\ref{lst:ge-qlx-p0}.  P1 places its persistent arithmetic
workspaces and typed CCZ-state stream on the selected board.  The QEC pipeline
lowers each Toffoli to a distance-27
surface-code consumer of an autocorrected CCZ resource, represented by the
implementation-specific type \texttt{AUTO\_CCZ\_STATE}; the physical pipeline
then materializes patch resources, native events, factory dependencies, and
timing at P3 before the generic scheduler constructs the event DAG.  Independently,
one complete factory lane---eight 15-to-1 protocols followed by CCZ and
autocorrection stages---is compiled and scheduled at P3.  That schedule has a
379-cycle empty-to-first-output latency, a 135-cycle steady-state cadence, and a
142,808-physical-qubit footprint.  The RSA device instantiates
the requested number of these characterized lanes.  With a $1\,\mu$s surface
cycle, distance 27, and a $10\,\mu$s reaction time,
CUDA-Q Logical \texttt{SCHEDULE} estimation reports time and occupancy from the verified schedule,
not from an algorithm-specific closed-form estimator.

% Listing~\ref{lst:ge-autoccz-factory} shows the typed factory composition,
% Listing~\ref{lst:ge-factory-characterization} derives its reusable model from
% the P3 schedule, and Listing~\ref{lst:ge-paper-device} binds the characterized
% lanes to the RSA device.  The complete P0-to-schedule path is summarized in
% Listing~\ref{lst:ge-p3-estimate}.

% May not need this one, doesn't fit well in the layout
% \begin{wrapfigure}{r}{0.50\textwidth}
%   \begin{minipage}{\linewidth}
% \begin{lstlisting}[
%   style=qlx-python,
%   % basicstyle=\scriptsize\ttfamily,
%   aboveskip=0pt,
%   belowskip=0pt,
%   caption={P0--P3 lowering and schedule-derived estimation for the selected RSA-2048 point.},
%   label={lst:ge-p3-estimate}
% ]
% p3 = ql.compile(rsa2048_resource_program
%     pipeline=ql.compiler.pipelines.physical(),
%     device=device)
% schedule = ql.compiler.schedule(p3)
% estimate = ql.estimate(
%     schedule, tier=ql.estimate.Tier.SCHEDULE,
%     p_phys=1.0e-3,
%     failure_budget=ql.estimate.FailureBudget(
%         total=0.8),
%     scaling=ql.estimate.Scaling(
%         prefactor=0.03, threshold=0.01),
%     cycle_time=1.0e-6,
%     evidence_policy=ql.estimate.EvidencePolicy())
% \end{lstlisting}
%   \end{minipage}
% \end{wrapfigure}


%Listing~\ref{lst:ge-p3-estimate} shows the complete P0-to-schedule path used
%for the sweep. It retains the scientific inputs and typed compiler boundaries
%while eliding routine helper and device-builder plumbing; the accompanying
%artifact contains the complete executable definitions.
Figure~\ref{fig:ge-factory-csep-sweep} varies the number of characterized
factory lanes for $c_{\mathrm{sep}}\in\{512,1024,2048\}$.  These separations
produce $(\text{pieces},\text{piece length})=(4,550)$, $(2,1062)$, and
$(1,2086)$, respectively.
With $c_{\mathrm{sep}}=512$, four carry pieces demand enough concurrent CCZ-state
supply that every sampled point from 8 through 40 factories remains
factory-limited.  Increasing the bank therefore continues to reduce the
single-run makespan from 12.995 to 4.147 hours.  With
$c_{\mathrm{sep}}=1024$, the two-piece adder crosses
from factory-limited to reaction/code-depth limited at 28 factories; the
makespan then saturates at 5.046 hours.  With $c_{\mathrm{sep}}=2048$, there is
no carry-piece parallelism.
The continuous supply boundary is 14 factories, and the sampled sweep first
shows the plateau at 16: all points from 16 through 40 remain at 7.925 hours.
Beyond these supply crossovers, reaction latency and code depth limit the
schedule; additional factories increase the physical-qubit footprint without
reducing the runtime. The default-point compiler result
and an independent source-model calculation are compared in
Table~\ref{tab:ge-reconciliation}.  Its folded P3 schedule contains 19,226
rows. 
Unlike quantities reported by the original analytical model, this value emerges directly from compilation and therefore remains attributable to the architectural and scheduling decisions encoded in the compiler artifact.

Together, these results show that CUDA-Q Logical can reproduce the RSA-2048
resource-analysis workflow as an inspectable compiler pipeline rather than as
a standalone resource estimate.  Because the compiled schedules preserve
attribution to the workload and architecture, the same model also reveals that
factory provisioning cannot be optimized independently of algorithmic
parallelism.  Below the supply crossover, additional factories reduce runtime;
above it, reaction latency and code depth dominate, so additional factories
only increase the physical-qubit footprint.


% \begin{table}[h]
%   \centering
%   \caption{Default-point reconciliation at $c_{\mathrm{sep}}=1024$ and 28
%     factory lanes. The independent column reconstructs only quantities
%     defined by the source model; compiler-internal schedule structure is
%     reported separately in the text.}
%   \label{tab:ge-reconciliation}
%   \small
%   \begin{tabular}{@{}lrr@{}}
%     \toprule
%     Quantity & CUDA-Q Logical schedule & Independent reconstruction \\
%     \midrule
%     Wall-clock time (h) & 5.046228 & 5.046228 \\
%     \midrule
%     Physical qubits & 19,252,128 & $19{,}248{,}768 + 28 \times 120$ \\
%     \bottomrule
%   \end{tabular}
% \end{table}

% \newpage
% \begin{lstlisting}[
%     style=qlx-python,
%     caption={The resource-faithful RSA-2048 arithmetic authored directly at CUDA-Q Logical P0.},
%     label={lst:ge-qlx-p0}
%   ]
%   def lookup_addition(_iteration, *live):
%       accumulator, address, bus, runways, \
%           ancillas, unlookup_access = split_workspace(live)

%       for row in range(1023):
%           address[row % 10], ancillas[0], \
%               ancillas[1], bus[row % 2124] = \
%               qrom_access_step(
%                   address[row % 10],
%                   ancillas[0],
%                   ancillas[1],
%                   bus[row % 2124])

%       accumulator, bus, runways = carry_runway_add(
%           accumulator, bus, runways,
%           piece_length=1062)

%       for fixup in range(64):
%           address[fixup % 10], ancillas[0], \
%               ancillas[1], unlookup_access = \
%               qrom_access_step(
%                   address[fixup % 10],
%                   ancillas[0],
%                   ancillas[1],
%                   unlookup_access)

%       return flatten_workspace(
%           accumulator, address, bus, runways,
%           ancillas, unlookup_access)


%   @ql.program
%   def rsa2048_resource_program() -> None:
%       accumulator = ql.allocate(2124, name="accumulator")
%       address = ql.allocate(
%           10, state=ql.types.plus, name="address")
%       bus = ql.allocate(2124, name="lookup_bus")
%       runways = ql.allocate(2, name="runways")
%       ancillas = ql.allocate(2, name="ancillas")
%       unlookup_access = ql.allocate(
%           1, name="unlookup_access")[0]

%       live = flatten_workspace(
%           accumulator, address, bus, runways,
%           ancillas, unlookup_access)
%       live = ql.ops.repeat(
%           505965,
%           carries=live,
%           body=lookup_addition)

%       accumulator, address, bus, runways, \
%           ancillas, unlookup_access = split_workspace(live)

%       for value in bus:
%           ql.measure_x(value)
%       for value in address:
%           ql.measure_x(value)
%       for value in runways:
%           ql.measure_z(value)
%       for value in ancillas:
%           ql.measure_z(value)
%       ql.measure_z(unlookup_access)
%       ql.measure_x(accumulator[0])
%       ql.discard(accumulator[1:])
%   \end{lstlisting}

%   \begin{lstlisting}[
%     style=qlx-python,
%     caption={Typed composition of the CCZ and AutoCCZ factory stages.},
%     label={lst:ge-autoccz-factory}
%   ]
%   @ql.protocol(
%       implements=ql.logical.produce(
%           ql.standard.CCZ_STATE))
%   def surface_ccz_8to1():
%       distilled_t = tuple(
%           surface_distill_15to1() for _ in range(8))
%       # Apply the checked CCZ circuit, postselection,
%       # and compiler-visible Pauli corrections.
%       ...
%       return ql.ops.pack_resource(
%           outputs, kind=ql.standard.CCZ_STATE)


%   @ql.protocol(
%       implements=ql.logical.produce(
%           ql.standard.AUTO_CCZ_STATE))
%   def surface_autoccz_factory():
%       ccz_state = surface_ccz_8to1()
%       _, main = ql.ops.unpack_resource(
%           ccz_state, like=main_anchors,
%           logical_ports=((0,), (0,), (0,)))

%       ring = build_nine_patch_ring(main, routing)
%       for matching in ((0, 3, 6), (1, 4, 7),
%                        (2, 5, 8)):
%           apply_ring_matching(ring, matching)

%       return ql.ops.pack_resource(
%           ordered_payloads(ring),
%           kind=ql.standard.AUTO_CCZ_STATE)
%   \end{lstlisting}

%   \begin{lstlisting}[
%     style=qlx-python,
%     caption={The reusable factory model is derived from a compiled P3 schedule.},
%     label={lst:ge-factory-characterization}
%   ]
%   factory_p3 = ql.compile(
%       surface_autoccz_factory,
%       pipeline=ql.compiler.pipelines.physical(),
%       device=detailed_factory_device)

%   factory_schedule = ql.compiler.schedule(factory_p3)

%   factory_estimate = ql.estimate(
%       factory_schedule,
%       tier=ql.estimate.Tier.SCHEDULE,
%       p_phys=1.0e-3,
%       failure_budget=0.8,
%       scaling=ql.estimate.Scaling(
%           prefactor=0.03, threshold=0.01),
%       cycle_time=1.0e-6)

%   factory_model = ql.compiler.factory_model(
%       factory_schedule,
%       produces=ql.standard.AUTO_CCZ_STATE)
%   \end{lstlisting}

%   \begin{lstlisting}[
%     style=qlx-python,
%     caption={The RSA device binds 28 lanes of the compiler-characterized factory.},
%     label={lst:ge-paper-device}
%   ]
%   factory = builder.logical.add_factory(
%       produces=ql.standard.AUTO_CCZ_STATE,
%       via=surface_autoccz_factory,
%       capacity=28,
%       name="autoccz_factory",
%       stream_name="autoccz_states")

%   factory_qec = builder.qec.bind(
%       factory,
%       encoding=surface_code,
%       block_capacity=9 * 28)

%   factory_lanes = builder.physical.add_resources(
%       "autoccz_factory_lane",
%       28,
%       name="factory_lanes",
%       granularity=ql.architecture.ResourceGranularity.PATCH,
%       footprint=ql.architecture.PhysicalFootprint(
%           factory_model.characterization.physical_unit_kind,
%           factory_model.characterization.physical_units,
%           "compiler-characterized AutoCCZ P3 schedule"))

%   builder.physical.bind(
%       factory_qec,
%       to=factory_lanes,
%       factory_model=factory_model)

%   device = builder.build()
%   \end{lstlisting}

%   \begin{lstlisting}[
%     style=qlx-python,
%     caption={Direct CUDA-Q Logical P0 progressively lowered to a schedule-derived estimate.},
%     label={lst:ge-p3-estimate}
%   ]
%   p0 = ql.compile(rsa2048_resource_program)
%   p1 = ql.compiler.place(p0, device=device)
%   p2 = ql.compile(
%       p1,
%       pipeline=ql.compiler.pipelines.qec(),
%       device=device)
%   p3 = ql.compile(
%       p2,
%       pipeline=ql.compiler.pipelines.physical(),
%       device=device)

%   schedule = ql.compiler.schedule(p3)
%   estimate = ql.estimate(
%       schedule,
%       tier=ql.estimate.Tier.SCHEDULE,
%       p_phys=1.0e-3,
%       failure_budget=0.8,
%       scaling=ql.estimate.Scaling(
%           prefactor=0.03, threshold=0.01),
%       cycle_time=1.0e-6)
%   \end{lstlisting}


%   \begin{lstlisting}[
%     style=qlx-python,
%     caption={Independent reconciliation of the compiler result with the source model.},
%     label={lst:ge-reconciliation}
%   ]
%   assert estimate.makespan_ns == schedule.makespan_ns
%   assert estimate.event_count == 19_226

%   paper_board_qubits = 19_248_768
%   explicit_injection_qubits = 28 * 120

%   assert estimate.physical_qubits == (
%       paper_board_qubits + explicit_injection_qubits)
%   assert estimate.physical_qubits == 19_252_128

%   compiler_hours = estimate.makespan_ns / 3.6e12
%   assert math.isclose(
%       compiler_hours, 5.046227985694444)
%   \end{lstlisting}



